When Benchmarks Talk: Re-Evaluating Code LLMs with Interactive Feedback

Programming is a fundamentally interactive process, yet coding assistants are often evaluated using static benchmarks that fail to measure how well models collaborate with users. We introduce an interactive evaluation pipeline to examine how LLMs incorporate different types of feedback in a collaborative setting. Specifically, we perturb static coding benchmarks so that the code model must interact with a simulated user to retrieve key information about the problem. We find that interaction significantly affects model performance, as the relative rankings of 10 models across 3 datasets often vary between static and interactive settings, despite models being fairly robust to feedback that contains errors. We also observe that even when different feedback types are equally effective with respect to performance, they can impact model behaviors such as (1) how models respond to higher- vs. lower-quality feedback and (2) whether models prioritize aesthetic vs. functional edits. Our work aims to "re-evaluate" model coding capabilities through an interactive lens toward bridging the gap between existing evaluations and real-world usage.

==> figtext/apps_interview_vanilla_baseline_best.tex <==
\begin{figure}[t]
    % \centering
    % \begin{subfigure}{.5\textwidth}
    \includegraphics[width=0.98\columnwidth]{figs/apps_interview_vanilla_baseline_best.pdf}
    % \end{subfigure}
    % \begin{subfigure}{.5\textwidth}
    %    \exampletable
    % \end{subfigure}
    \caption{
        Comparison between different settings on APPS (Interview). \jane{is this not aggregated across datasets?} The average test case accuracy drops significantly in the \baseline{} setting compared to the \vanilla{} setting, showing the effects of underspecification.
        The test case accuracy is recovered with iterative refinement, showing that \user{} feedback can improve on the \vanilla{} setting.
    }
    \vspace{-5pt}
    
    \label{fig:vanilla_baseline}
\end{figure}


==> figtext/role_of_user.tex <==
\begin{figure*}[ht]
    \centering
    % \begin{subfigure}{.5\textwidth}
    \includegraphics[width=1\textwidth]{figs/role_of_user_TEMP.png}
    % \end{subfigure}
    % \begin{subfigure}{.5\textwidth}
    %    \exampletable
    % \end{subfigure}
    \caption{
        \redtext{TODO}
    }
    \vspace{-5pt}
    \label{fig:role_of_user}
\end{figure*}


==> figtext/steerability_vs_perf_delta.tex <==
\begin{figure*}[ht]
    \centering
    % \begin{subfigure}{.5\textwidth}
    \includegraphics[width=0.98\textwidth]{figs/edit_distance_vs_steerability_heatmap.png}
    % \end{subfigure}
    % \begin{subfigure}{.5\textwidth}
    %    \exampletable
    % \end{subfigure}
    \caption{
        \redtext{TODO: write caption}
    }
    \vspace{-5pt}
    
    \label{fig:edit_distance_vs_steerability_heatmap}
\end{figure*}


==> figtext/vanilla_baseline_barplot.tex <==
\begin{figure}[t]
    % \centering
    % \begin{subfigure}{.5\textwidth}
    \includegraphics[width=0.98\columnwidth]{figs/all_datasets_best_feedback.pdf}
    \caption{
        Comparison between \vanilla, \baseline, and the best-performing interactive feedback type aggregated across datasets. The performance drops significantly in the \baseline{} setting compared to the \vanilla{} setting but recovers with feedback, showing that collaboration with the \user{} is required for performance on obfuscated inputs to be comparable with the \vanilla{} setting.
    }
    \vspace{-5pt}
    
    \label{fig:vanilla_baseline}
\end{figure}


==> sections/1_a_introduction.tex <==



\section{Introduction}

\val{add cites throughout}

Human (or even LLM-based) feedback is increasingly used for reward modeling and aligning large language models (LLMs) with downstream tasks. 
While feedback is important in the model training process, these models are increasingly also deployed at test time, encountering varying forms of feedback.
Understanding how models incorporate feedback is relevant in multi-agent systems, where the ``orchestrator'' may delegate sub-tasks to specialized agents and provide feedback on that agent's progress.
Humans also increasingly interact with and provide feedback to LLMs, where chat interfaces like ChatGPT facilitate multi-turn conversations in which humans can iteratively refine the task they want to accomplish using LLMs.
Across these use cases, there is no form of feedback that has been established as optimal.
In this work, we ask: \textit{how well do LLMs incorporate different forms of feedback?}

Programming applications are the focus of our work, and are a setting where one might find multiple forms of feedback.
Programming with an assistant is a highly collaborative task where the user and model develop a solution together.
For example, one increasingly common workflow is to iterate with a chat-based coding assistant to build and refine code, where refinement steps involve users correcting specific code or writing natural language to change the code functionality. 
Despite the popularity of these tools---millions of developers use Github Copilot---existing
evaluations of the coding capabilities of new models fail to capture these interactive settings.
Existing benchmarks rely on a simple input-output configuration, where the question and provided code are fully provided and the model is asked to generate the whole completion in one shot. 
Existing benchmarks also assume that the input is well-specified and error-free, further reducing the need for interactive feedback.

% In order to complete a provided code snippet, models must correctly infer the full user intent---i.e., the function that the user wants to implement via the code, and potentially rely on explicit human feedback to steer model generation.
 


% Not only do code benchmarks not properly simulate realistic programming settings, but they also avoid other critical questions that arise as a result of model-user interaction. For instance, in practice, users do not usually accept large blocks of model-generated code -- they may delete a significant portion of the generation and insert their own code or comments. In doing so, they are implicitly performing a variation of \textbf{mid-generation guidance}, in which the user intervenes midway through a model generation. Explicitly examining this setting for a code model raises several key questions. For instance, when should a user intervene? Can models identify when they require more information from the user and query them for mid-generation guidance? 

% Since this aspect of the coding process is understudied, most users of code assistants do not trust models to make changes on a larger-than-local level. Programmers usually allow models to generate just a few lines of code, which can be easily manually checked for correctness. This limits the utility of code assistants in a practical setting as programmers cannot rely on models to correctly generate longer completions.


% In order to complete a provided code snippet, models must correctly infer the \textbf{user intent} -- the function that the user wants to implement via the code. This process is usually done \textit{implicitly}, i.e. the model directly generates a code completion that implements the user's desired function. Meanwhile, user-provided \textit{explicit} statements of intent (including function docstrings or comments) can be critical to steering model generation. If they are provided by the user, they are usually provided once, i.e. before the generation. Moreover, while high-level intent may be clear from a provided docstring, unforeseen choices (e.g. over edge cases or what variables to optimize) may remain ambiguous.


% Currently, most users of code assistants do not trust models to make changes on a larger-than-local level. Programmers usually allow models to generate just a few lines of code, which can be easily manually checked for correctness. However, when coding assistants are allowed to generate larger amounts of code, programmers often find that the code is buggy or does not implement the precise functionality that the programmer intended. This limits the utility of code assistants in a practical setting as programmers cannot rely on models to correctly generate longer completions.

In this work, we study how code models perform under more realistic user interactions.
We propose an evaluation method that transforms a generic coding benchmark into one that incorporates underspecification and human feedback. 
Specifically, given a code dataset with well-specified problems, test cases, and at least one ground-truth solution, we introduce a pipeline that creates under- or misspecified problems and a simulated user who can be queried for guidance, with a variety of feedback formats.
The goal is to capture characteristics of real code repositories and interactions with programmers that may include underspecified problems (e.g. over edge cases or what variables to optimize) in the form of function docstrings or comments.
We explore multiple formats including user-written comments, code, and user selection of model-generated multiple-choice answers to a model-generated question.


Across 9 models and 3 coding benchmarks, we find multiple insights.
\val{just copied directly from gdoc:} Models that perform similarly on static coding benchmarks often perform differently in the collaborative setting; on the other hand, models that perform differently on static coding benchmarks may perform similarly in a collaborative setting.
Models vary in terms of which feedback type is most effective.
Question difficulty (and other question-specific aspects??) affect how models incorporate feedback.
Feedback quality affects how the model affects feedback.
\val{Need to give more specific examples once we have a draft of results in, Talk about findings and implications for future design of coding assistants.}



% \begin{itemize}
%     \item \textbf{A plug-and-play pipeline.} Our code is designed to easily integrate with any code benchmark.
%     \item \textbf{Input perturbation to simulate under- or misspecification of problems.} 
%     \item \textbf{A simulated user who can be queried for guidance, with a variety of feedback formats.} Formats include user-written comments, user-written code, and user selection of model-generated multiple-choice answers to a model-generated question.
%     \item \textbf{Multiple settings for incorporating user feedback.} User guidance can be introduced via both iterative refinement and mid-generation guidance. In the latter, a heuristic must be applied to guide when the model pauses to allow user intervention.
% \end{itemize}


\begin{comment}
\begin{enumerate}
    \item What kind of task description errors are realistic?
    \begin{enumerate}
        \item Typically, errors in the input can be categorized as underspecification (via missing information or ambiguity), misspecification (via erroneous instructions), or a combination of both.
    \end{enumerate}
    \item How do we simulate feedback from a human, and what forms can this take?
    \begin{enumerate}
        \item 
    \end{enumerate}
    \item{What mode of incorporating user feedback have the best effects on performance and efficiency?}
\end{enumerate}
\end{comment}


==> sections/2_problem_def.tex <==

\section{General Problem Formulation}

We first describe the general problem formulation of humans interacting with AI assistants, and later propose an evaluation pipeline to study the problem in detail through the lens of coding assistants.

\begin{itemize}
    \item Given an underspecified problem, there are multiple possible implementations that satisfy the set of criteria put forth by the current problem definition
    \item Conditions:
    \begin{itemize}
        \item Assistant alone (and self-critique)
        \item Assistant + human: 
    \end{itemize}
    \item Evaluation: Solution is evaluated via a function. In addition we might care about the human effort required.
\end{itemize}

==> sections/4_results_OLD.tex <==


\section{Results}
We discuss the overall trends in model behavior when comparing static to interactive settings. \val{mention focus on feedback types}


\input{figtext/edit_distance_vs_steerability_ranking}

\subsection{General trends in model behavior}
Figure \ref{fig:ranking_changes} shows our main results using all \nmodels{} models on the three datasets: APPS, LiveCodeBench, and ClassEval.
The plot shows the relative rankings of each model (measured by their test case accuracy on each dataset) on each of the settings: \vanilla, \para, \sent, \cf, and \ir.

\paragraph{Relative performance between models change between different static and interactive settings.} 
Figure \ref{fig:ranking_changes} shows that the rankings of models often vary depending on which setting is being used to evaluate performance. 
% While \qwenSmall{} performs third in \vanilla{} for LiveCodeBench, it falls to fifth in other feedback settings, and even seventh in \cf. 
% \gemmaLarge{} performs fifth in \vanilla{} and even falls to seventh in \ir, yet jumps to third in \para. \sonnet{} beats \gpt{} in all settings of APPS Interview, except for \cf, where their order inverts.
Tables \jane{ref} shows the normalized Spearman Footrule distances ($\tilde{F})$ between the \vanilla{} and interactive settings. 
It is clear that the choice of evaluation setting has a profound impact on the relative performance of models. 
For ClassEval, $\tilde{F}$ ranges from $0.98$ to $0.67$, indicating anti-correlation between the \vanilla{} and interactive settings.
LiveCodeBench and APPS also demonstrate relatively weak positive correlation on many interactive settings; for instance, for \cf, $\tilde{F}$ is $0.36$ and $0.26$, respectively.
For these two datasets, top models tend to be more consistent, preserving their positions in high positions, whereas weaker models tend to demonstrate more variance in rank.
%\val{i think we should talk about top models being more consistent even with feedback}


% \val{add another paragraph to talk about which feedback types are most helpful}

\paragraph{Dataset difficulty correlates with ranking.}
\jane{Help}

\paragraph{Underspecification hurts model performance, and performance is recoverable only with the incorporation of feedback.}

Figure \ref{fig:vanilla_baseline} plots the best feedback setting for each model, as well as its performance on the \baseline{} and \vanilla{} settings. 
Comparing the blue bars (\vanilla) to the orange bars (\baseline), it is clear that our input perturbation successfully underspecifies the problem, as \baseline{}  consistently underperforms the \vanilla{} setting. 
In order to recover performance comparable with the \vanilla{} setting, the models must interact with the \user{} (as in the \para, \sent, \cf, and \ir{} settings).

\paragraph{\cf{} and \para{} boost performance the most.}


\subsection{Effect of Feedback Quality}
We examine the effects of the feedback type and quality level on performance. \val{provide some intuition for why we look at this}


\paragraph{Feedback quality is consistent across models.}
Table \ref{tab:feedback_quality_max_step_number} compares average feedback quality and the average maximum number of steps.
The feedback quality does not vary greatly across models and often falls above $0.9$.
This suggests that the feedback is high-quality enough to be compared across models on different trajectories of iterative refinement. 
\jane{See HH's comment. Not sure if I captured this sensibly.}

We note that our metric of feedback quality does not correlate with a reduction of the average maximum number of steps ($r=0.48$).
Rather, the maximum number of steps seems to be more related to feedback type, as \cf{} consistently has the the smallest maximum step number, followed by \para{} and \sent.

Surprisingly, when \sonnet{} is the \cm{}, it receives the worst quality feedback compared to the other models, despite being both the \cm{} and the \user{}. 
However, it still completes the solutions the fastest, and consistently has the lowest average maximum step number compared to \gpt{} and \sonnet. 


\paragraph{Code models are robust to \lqf{} feedback.}
Figure~\ref{fig:effect_of_fq} shows the distribution of solutions whose performances improve, do not change, or decrease when comparing \hqf{} feedback to \lqf{} feedback. 
High quality feedback reduces the proportion of feedback that does not have an effect on the solution.
This usually results in a higher rate of solutions whose performances are improved.
\textsc{high-quality} \sent{} feedback usually decreases the rate of worse solutions.
Interestingly, while \cf{} often increases the proportion of improved solutions more than \para{} or \sent, it almost always increases the proportion of worse solutions.




%\paragraph{Average feedback quality varies per feedback type.} 
%\val{this takeaway is weak}


\input{figtext/edit_distance_vs_steerability_heatmap}


\subsection{Effect of Feedback Type and Code Model Steerability}

\val{reframe as how models respond to feedback, rename subsection}
The effects of feedback formats and quality level on surface-level and behavioral-level steerability.
In this section, we discuss how different aspects of feedback affect the \cm 's ability to change its previous version of the solution.

\paragraph{\para{} feedback is associated with higher steerability across all models.} 
Figure \ref{fig:edit_distance_vs_steerability_ranking} ranks each feedback type according to how behavioral (left) or surface-level (right) steerability it induces.
\para{} and \cf{} consistently rank the highest in behavioral steerability, ranking first and second, respectively. 
Likewise, \para{} and \sent{} rank the highest in surface-level steerability. 
This suggests that some feedback types tend to induce similar steerability relative to other feedback types on the same model.


\paragraph{Models react differently to the same forms of feedback, both in terms of behavioral- and surface-level steerability.} 
Figure \ref{fig:edit_distance_vs_steerability_heatmap} shows the effect of feedback type on how \cm s change their previous solutions for \gpt{} on APPS Interview.

Some models (e.g. \gemmaSmall{} or \reka) tend to make large number of surface-level changes that do not greatly affect the behavior of the language model.
Other models (e.g. \gpt{} or \sonnet, and \qwenLarge) demonstrate a bimodal distribution, where some edits highly affect code behavior and others do not.
% While \para{} has demonstrates bimodal 
Appendix \ref{app:extra_figs} shows additional tables and figures.

% Figure \ref{fig:steerability_vs_performance_delta} plots the changes in test cases against the change in performance on a step-by-step basis.
% Green points are code solutions where the last step had an improvement in performance; red points are code solutions where the last step did not have an improvement in performance.

% We note that while the first step has relatively few points with a decrease in performance, the following steps have increasingly high "tails" where changes in test case behavior are attributed to high attrition of performance.
% Moreover, these "tails" are predominantly made up of points where the last step had an improvement in performance.
% Because the interaction is generated in a history-less setting, this cannot be attributed to weaker performance induced by long conversation contexts.
% The tails are also present when history is included in the conversation, meaning that the tails also cannot be attributed to loss of information from lack of history. \redtext{Need to double check this!}
% More details about history and its effect on results can be found in \ref{app:ablations}.




==> tables/old_feedback_quality_max_step.tex <==

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccc}
\toprule 
\textbf{Feedback} & \textbf{Code Model}             & \textbf{Avg. Quality} & \textbf{Avg. Max Step} &  \\ \hline
              & \gpt            & 0.873                 & 3.983                &  \\
\textit{Paragraph}     & \deepseek & 0.869                 & 4.170                &  \\
              & \sonnet     & 0.796                 & 3.930                &  \\ \hline
              & \gpt            & 0.831                 & 4.490                &  \\
\textit{Sentence}      & \deepseek & 0.854                 & 4.467                &  \\
              & \sonnet     & 0.762                 & 4.293                &  \\ \hline
              & \gpt            & 0.948                 & 4.257                &  \\
\textit{Code Feedback} & \deepseek & 0.928                 & 4.207                &  \\
              & \sonnet     & 0.895                 & 4.240                & \\ \hline
\end{tabular}
}

\caption{
    \redtext{TODO} \val{can we show quality high across datasets?}
    }
    \label{tab:feedback_quality_max_step_number}
\end{table}

